Commitment Attacks on Ethereum's Reward Mechanism

Validators in permissionless, large-scale blockchains, such as Ethereum, are typically payoff-maximizing, rational actors. Ethereum relies on in-protocol incentives, like rewards for correct and timely votes, to induce honest behavior and secure the blockchain. However, external incentives, such as the block proposer's opportunity to capture maximal extractable value (MEV), may tempt validators to deviate from honest protocol participation. We show a series of commitment attacks on LMD GHOST, a core part of Ethereum's consensus mechanism. We demonstrate how a single adversarial block proposer can orchestrate long-range chain reorganizations by manipulating Ethereum's reward system for timely votes. These attacks disrupt the intended balance of power between proposers and voters: by leveraging credible threats, the adversarial proposer can coerce voters from previous slots into supporting blocks that conflict with the honest chain, enabling a chain reorganization. In response, we introduce a novel reward mechanism that restores the voters' role as a check against proposer power. Our proposed mitigation is fairer and more decentralized, not only in the context of these attacks, but also practical for implementation in Ethereum.

==> fixed_validator_set.tex <==
\section{Attacks in the Presence of a Fixed Attestor Set}
\label{sec:fixed-validator-set}
% 
In Sections~\ref{sec:solo-validators-simple} and~\ref{sec:solo-validators-extended}, we have analyzed the simple and the extended attacks under 2 assumptions: i) all attestors are solo validators, and ii) the attestor set is different in each slot.
This matches the current version of Ethereum, where
% in each epoch consisting of 32 slots, 
the validators are divided into $32$ attestor committees, each for a different slot. 
% This implies that the attestor set is rotated in each slot of the current Ethereum version. 
% However, once Ethereum adopts single-slot finality, where a block is proposed and finalized in the same slot, all attestors would need to send a vote in each slot. 
% Therefore, 
% in a protocol with single-slot finality, we expect to have a fixed set of attestors across slots. 
In this section, we analyze the simple and the extended attacks assuming the same set of attestors across slots.
% under the assumption that the attestor set across slots is fixed. 
This analysis serves a dual purpose. 
First, it shows that our attacks apply to Ethereum with single-slot finality~\cite{singleSlotFinality}, where all attestors send votes in each slot, and to other similar protocols featuring a fixed attestor set. 
%(whereas the extended attack fails). 
Second, it demonstrates the success of the attacks 
% enables us to analyze these attacks 
in the presence of staking pools.
% which are modeled as single entities controlling a fixed number of votes in each slot.
% A staking pool is defined as a set of colluding validators across slots.
% % under the fixed validator set model\footnote{
% Thus, we model a staking pool as a single entity controling a fixed number of votes in each slot.
% }.
 
A fixed validator set can influence the strategy of a rational attestor against the attack.
Indeed, 
% consider the simple game, where slot $t+1$ is adversarial. 
for analyzing the simple game under rotating attestors, we only had to consider the head vote reward of a solo validator for its vote in slot $t$.
However, under a fixed attestor set, we should consider the reward an attestor receives in both slots $t-1$ and $t$. 
This is because if the adversary reorgs the block of slot $t$, the slot $t-1$ reward is affected as well.

\subsection{The Simple Game}
\label{sec:fixed-validator-set-simple-game}
% 
The simple game and the adversarial action are the same as in Section~\ref{sec:simple-game} except that a solo validator $\val$'s payoff depends on its votes in each of the slots $t-1$ and $t$.

\begin{theorem}
\label{thm:fixed-validator-set-simple-game-theorem}
There exists a Nash equilibrium of the simple game 
% in the presence of solo validators 
under the fixed validator set model, where the adversary succeeds.
% with $\br = 0$ budget.
\end{theorem}
% 
Proof of Theorem~\ref{thm:fixed-validator-set-simple-game-theorem} for a fixed set of \emph{solo} validators is presented in Appendix~\ref{sec:appendix-proof-simple-game-fixed}. Fig.~\ref{fig:simple_game_staking_pool} illustrates the intuition behind the proof.

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[height=1.2in]{Pic3.jpg}
        \caption{$\texttt{Fail}$, $NC_P$. The payoff of staking pool $P$ is equal to $mr$.}
        \label{fig:simple_game_staking_valool_AV}
    \end{subfigure}%
    ~ 
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[height=1.2in]{Pic4.jpg}
        \caption{$\texttt{Fail}$, $C_P$. The payoff of staking pool $P$ is equal to $mr$.}
        \label{fig:simple_game__staking_valool_ANV}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[height=1.2in]{Pic5.jpg}
        \caption{$\texttt{Succeed}$, $NC_P$. The payoff of staking pool $P$ is equal to $0$.}
        \label{fig: simple_game__staking_valool_NAV}
    \end{subfigure}
    ~ 
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[height=1.2in]{Pic6.jpg}
        \caption{$\texttt{Succeed}$, $C_P$. The payoff of staking pool $P$ is equal to $mr$.}
        \label{fig:simple_game_staking_valool_NANV}
    \end{subfigure}%
    \caption{The payoff of a staking pool $P$ with a total stake share less than $\Wp$ in the simple game under the fixed validator set model. The staking pool $P$ controls $m$ votes in each slot, where $m$ can be either 1 (representing a solo validator) or greater than 1 (representing a coalition of solo validators). $r$ represents the reward for a single correct and timely head vote. Let $C_P$ and $NC_P$ denote the events that the staking pool $P$ votes and does not vote for $B_{t-1}$ (acts compliantly and non-compliantly), respectively. Let $\texttt{Succeed}$ denote the event that less than $\Wp$ slot $t$ attestors vote for $B_t$ (the attack succeeds), and $\texttt{Fail}$ the event that $\Wp$ or more slot $t$ attestors vote for $B_t$ (the attack fails). The green tick and the red cross represent whether a head vote receives or does not receive a reward, respectively. As can be seen, $C_P$ (compliance) weakly dominates $NC_P$ (non-compliance).}
    \label{fig:simple_game_staking_pool}
\end{figure*}

\begin{note}
There are Nash equilibria, similar to those in Note~\ref{note:4.1}, where the adversary $\mathcal{A}$ is not successful. 
As in Notes~\ref{note:4.2} and~\ref{note:4.3}, $\mathcal{A}$ can ensure its success in \emph{all} Nash equilibria by offering an $\epsilon/W$ amount of bribe to each slot $t$ attestor to vote for $B_{t-1}$, and given an honest minority, there is a Nash equilibrium where the adversary succeeds.
\end{note}

% \begin{note}
% If the staking pool $\val$ controls over $\Wp$ attestors per slot, payoff of the $NA - V_\val$ corner becomes $mr+0$ for $\val$ in Table~\ref{table:pay-off-matrix_simple-game_staking-pool}.
% Then, voting for block $B_t$ at slot $t$ weakly dominates voting for $B_{t-1}$ for $\val$, given any actions by the other attestors.
% If $\val$ votes for $B_t$, $\mathcal{A}$ cannot reorg $B_t$ with its block $B_A$, \ie, is unsuccessful.
% \end{note}

\subsection{The Extended Game}
\label{sec:fixed-validator-set-extended-game}
The extended game and the adversarial action are the same as in Section~\ref{sec:solo-validators-extended} except that a solo validator's payoff depends on its votes in each of the slots.
% This makes the extended game a \emph{repeated game}.
% and the correct notion of equilibria, the subgame-perfect Nash equilibrium.
% We again assume that the staking pool does not control any of the leaders for slots in $[p]$.
% 
\begin{theorem}
\label{thm:fixed-validator-set-extended-game-theorem}
There exists a SPNE of the extended game 
% in the presence of solo validators 
under the fixed validator set model, where the adversary succeeds 
% with $\br = 0$ budget 
and violates the security of LMD GHOST.
\end{theorem}
% 
Proof of Theorem~\ref{thm:fixed-validator-set-extended-game-theorem} is in Appendix~\ref{sec:appendix-proof-extended-game-fixed} and has a similar outline as the proof of Theorem~\ref{thm:repeated-game-theorem}.
% and is presented below.
% % Since the staking pool controls less than $\Wp$ attestors per slot, it has the same payoff table for the attestation rewards of each slot $i \in [p]$ as Tables~\ref{table:payoff_matrix-repeated_game_\val} and~\ref{table:payoff_matrix-repeated_game_i}.

\begin{note}
\label{note:extended_game_fixed_validator}
% There are subgame perfect Nash equilibria, similar to those in Section~\ref{sec:solo-validators-extended}, where the adversary $\mathcal{A}$ is not successful.
There are SPNE, similar to those in Note~\ref{note:5}, where the adversary $\mathcal{A}$ is not successful.
However, unlike in Note~\ref{note:5}, $\mathcal{A}$ cannot ensure its success in all SPNE by offering a small bribe to the attestors to send compliant votes.
Suppose all leaders and attestors of slots $1, \ldots, p$ extend a chain from block $B_0$ instead of attempting to reorg the blocks from slots $-p+1, \ldots, 0$.
This is a SPNE, where the attestors' total payoff during the $2p+1$ slots within $[-p,p]$ is $2pr > pr$, and the adversary cannot convince any attestor to deviate if its total budget is less than $r$.
% However, $\mathcal{A}$ can again ensure its success in \emph{all} subgame perfect Nash equilibria by offering an $\epsilon/pW$ amount of bribe to each slot $t$ attestor to send compliant votes.
As in Note~\ref{note:5}, under an honest minority assumption, there is still a SPNE where the adversary succeeds.
\end{note}

% Although the extended game under the fixed validator set model results in a subgame perfect Nash equilibrium where the adversary succeeds, 
% The extended attack is unlikely to be successful in practice as there are other equilibria such as the one presented in Note~\ref{note:extended_game_fixed_validator}, where the validators achieve greater payoffs compared to the equilibrium of the successful extended attack.
%due to two reasons:
% Here, we outline 2 justifications for the attack's possible failure in reality:

% For instance, consider the equilibrium example presented in Note~\ref{note:extended_game_fixed_validator}. 
% This equilibrium provides a greater payoff for the leaders and attestors of slots $1, \ldots, p$ 

% For instance, consider the extended game that starts at slot $t$ and aims to reorg blocks $B_i, \enspace i \in \{t-p+1, \cdots, t\}$ using blocks $B_j, \enspace j \in \{t+1, \cdots, t+p\}$. 
% If all players follow the game rules and the attack succeeds, a slot leader receives the inclusion reward, and an attestor receives $pr$ head vote rewards during interval $\{t-p, \cdots, t+p\}$. 
% However, if they all follow the honest protocol, a slot leader receives both the transaction and inclusion rewards and an attestor receives $2pr$ head vote rewards during the interval $\{t-p, \cdots, t+p\}$ (only missing the head vote reward of the slot preceding the adversarial slot). 
The existence of equilibria as in Note~\ref{note:extended_game_fixed_validator}, where the attestors achieve greater payoffs compared to the SPNE of the attack 
% with greater payoffs 
incentivizes them to 
% coordinate their strategies or 
collude as a single entity (\eg, a staking pool) to mitigate the attack. 
% Second, following the extended game rules can dominate behaving non-compliantly for a player only if its subsequent players are payoff-maximizing validators. 
% Even the existence of an honest minority (an honest slot leader) can affect the rational validators' strategy, resulting in the attack's failure.
% 
% An adversary faced with colluding attestors may refer to the \emph{selfish mining-inspired attack} in Appendix~\ref{sec:fixed-validator-set-selfish_mining_game}, which achieves adversarial success under more practical assumptions, albeit under higher requirements of control over slots. There, even colluding validators are incentivized to comply with the adversary.
An adversary faced with colluding attestors may refer to the \emph{selfish mining-inspired attack} in Appendix~\ref{sec:fixed-validator-set-selfish_mining_game}, where even colluding validators are incentivized to comply with the adversary.
% However, this attack requires higher adversarial control over slots.
However, this attack requires a larger stake share.

\subsection{Attacks in the Presence of Staking Pools}
\label{sec:selfish_mining_game}
% Recall that a staking pool is defined as a set of colluding solo validators under the fixed validator set model (\cf Section~\ref{sec:model}). 
% This definition implies that a staking pool controls a fixed number of attestors, denoted by $m$, in each slot.
% Recall that a staking pool was defined as a set of colluding validators across slots (\cf Section~\ref{sec:model}).
% under the fixed validator set model\footnote{
% Thus, we model 
A staking pool is modelled as a single entity controlling a fixed number of votes in each slot.
If a staking pool $P$ controls less than $\Wp$ attestors per slot, acting compliantly (voting for $B_{t-1}$) weakly dominates any other action in the simple game as shown on Fig.~\ref{fig:simple_game_staking_pool}.
On the other hand, if $P$ controls over $\Wp$ attestors\footnote{As of May 20, 2024, the largest staking pool is LIDO, holding $28\%<\Wp = \%40$ of the total Ethereum stake~\cite{lido}.} per slot, acting non-compliantly (voting for $B_{t}$) weakly dominates any other action in the simple game, even though following the adversarial action (voting for $B_{t-1}$) still remains weakly dominant.
Therefore, using the same analysis employed in the fixed validator set model (\cf Section~\ref{sec:fixed-validator-set-simple-game}, 
% \ref{sec:fixed-validator-set-extended-game}, 
and Appendix~\ref{sec:fixed-validator-set-selfish_mining_game}), we can establish the existence of Nash equilibria of the simple and selfish mining-inspired games in the presence of a staking pool \emph{with any size}, where the adversary succeeds.
% at no cost ($\br = 0$).
%D
This shows that the attacks could succeed even when the rational attestors collude.
% as long as the size of the colluding set is bounded by $\Wp$.

% \begin{note}
% If the staking pool $P$ controls over $\Wp$ attestors\footnote{Currently, the largest staking pool is LIDO, which holds $32\%$ of the total Ethereum stake~\cite{lido}, well below $\Wp = \%40$.} per slot, acting non-compliantly (voting for $B_{t}$) weakly dominates any other action in the simple game, even though following the adversarial action (voting for $B_{t-1}$) still remains weakly dominant.
% \end{note}

% \begin{note}
% The existence of a Nash equilibrium of the selfish mining-inspired game in the presence of staking pools implies that under the current Ethereum reward mechanism, none of the provably-secure alternatives to LMD GHOST that retain its slot based structure and heaviest-tree based fork-choice rule can offer greater security than the predictable longest-chain fork choice rule of Nakamoto consensus. 
% \end{note}

==> gasper-diagram.tex <==
\begin{tikzpicture}[x=1.5cm,y=0.62cm]
    % \footnotesize
    \scriptsize

    \node (txs) at (-1.75,0) {$\txs$};

    \node [draw,align=center,minimum width=2cm,minimum height=0.8cm] (lmdghost) at (-0.3,0) {LMD GHOST};

    \coordinate (logavailable) at (1,0) {};

    \node [draw,align=center,minimum width=2cm,minimum height=0.8cm] (casperffg) at (2.3,0) {Casper FFG};

    \coordinate (logaccountable) at (3.5,0) {};
    \coordinate (logaccountableOUT) at (5,0) {};

    \draw [-Latex] (txs) -- (lmdghost);
    \draw [-Latex] (lmdghost) -- (logavailable) node [above,pos=1,yshift=1pt] {Chain tip};
    \draw [-Latex] (logavailable) -- (casperffg);
    \draw [-Latex] (casperffg) -- (logaccountable);
    \draw [-Latex] (logaccountable) -- (logaccountableOUT) node [pos=1,above,align=right,anchor=south east,yshift=1pt] {Finalized Ledger};
    % node [pos=1,right] {$\chainacc$};
    \draw [-Latex] (logaccountable) -- ++(0,1.5) -- ++(-3.8,0) -- (lmdghost) node [pos=0.35,right] {Justifications};
    \draw [-Latex] (logavailable) -- ++(0,-0.9) -- ++(2,0) -- ++(2,0) node [pos=1,above,align=right,anchor=south east,yshift=1pt] {Available Ledger};
    %node [pos=1,right] {$\chainava$};
\end{tikzpicture}%

==> goldfish_new_mechanism.tex <==
\section{\NewMechanism Mechanism Proposed for Goldfish}
\label{sec:new-mechanism-goldfish}
% 
Goldfish satisfies reorg resilience, safety and liveness under the $\Delta$-synchronous sleepy network model~\cite{sleepy}
% network with delay upper bound $\Delta$ and unexpected temporary crash faults that can affect any fraction of the validators, 
and an honest majority among the awake validators~\cite[Section 4, Theorems 2 and 3]{d2022goldfish}.
The analysis in~\cite{d2022goldfish} does not consider rational validators or any reward mechanism; however, it is crucial to incentivize timely voting in Goldfish due to vote expiry.
If Ethereum's reward mechanism were to be applied for this purpose, such that a vote is rewarded if it is included by the next slot's block, the protocol would be susceptible to the same attacks.
% in Sections~\ref{sec:solo-validators-simple} and~\ref{sec:solo-validators-extended}.
% As in Section~\ref{sec:solo-validators-simple}, this enables an adversarial leader of a slot $t$ to reorg the slot $t-1$ block by committing to an action, where the slot $t-1$ votes are included in the proposed slot $t$ block only if they are for the \emph{parent} of the slot $t-1$ block.
% Extending this attack across multiple slots, the adversary can violate safety and liveness by committing to the action in Section~\ref{sec:solo-validators-extended}.
Thus, to retain security with rational validators, we adapt \newmechanism to Goldfish.
% in Section~\ref{sec:new-mechanism-ethereum} for Goldfish.

Each slot $t+1$ voter is asked to sign all slot $t$ votes it observes at time $4\Delta t + 2 = 4t + 2$, \ie, $2\Delta = 2$ time steps into slot $t$.
% (\ie, at time $3t+2$ for slots of size $3$).
A signature on a slot $t$ vote by a slot $t+1$ voter is again called a slot $t$ evidence.
A slot $t$ voter is rewarded within the canonical chain block $B$ with the smallest slot $t' > t+\kappa$, if its vote $v$ is \emph{correct} and \emph{timely} with respect to $B$:

\smallskip
\noindent
\textbf{Correctness:}
Let $B_l$ denote the block supported by the vote $v$.
The vote $v$ is correct if $B_l$ is of some slot $\leq t$ and the chains defined by $B_l$ and $B$ intersect at a block of slot $\geq t - \kappa$.
% it is for the highest block from slots $\leq t$ in the prefix of $B$ (let $B_\ell$ denote this block).

\smallskip
\noindent
\textbf{Timeliness:}
Let $W$ denote the number of unique slot $t+1$ voters such that at least one slot $t$ evidence by each voter is included in the prefix of $B$ after block $B_\ell$.
The vote $v$ is timely if either $v$ is included by a slot $t+1$ block in the prefix of $B$, or there are more than $W/2$ unique slot $t$ evidences for $v$ in the prefix of $B$ after block $B_\ell$.

\smallskip
Leaders can be rewarded for including in their blocks the votes and evidences that have not been captured by previous blocks to incentivize inclusion.
Similarly, for all $t$, the slot $t+1$ voters can be rewarded for each slot $t$ evidence on the vote of a unique slot $t$ voter, once the evidence is included in the canonical chain.
However, for simplicity, we do not consider these rewards in the subsequent analysis.

Note that there is a $\kappa$ difference between the slot ($t$), at which a slot $t$ evidence is created and the slot ($>t+\kappa$), at which the vote $v$ is rewarded.
This is to guarantee the existence of an honest leader that would include all evidences created by the slot $t+1$ voters on behalf of the vote $v$ revealed at the correct time.
Moreover, $v$'s timeliness is determined by the \emph{relative} number of evidences for that vote among the slot $t$ evidences, as opposed to an absolute number as in Section~\ref{sec:solution}.
This is because Goldfish is designed to remain secure under the sleepy network model and does not require a fixed threshold on the number of awake validators per slot.
To retain the same property, we ensure that a timely slot $t$ vote can be rewarded given any number of awake slot $t+1$ voters.

\subsection{Attacks on \NewMechanism Proposed for Goldfish}
\label{sec:liveness-attack-on-goldfish}

Despite mitigating the earlier attacks, 
% of the previous sections, 
\newmechanism cannot ensure security in all Nash equilibria.
Suppose the rational slot $i \in [\kappa]$ voters vote for the genesis block throughout the first $\kappa$ slots, while creating evidences for the previous slots' votes.
Then, the first $\kappa$ blocks do not receive any votes.
Subsequently, the slot $\kappa+1$ block reorgs the first $\kappa$ blocks and includes all of the slot $i \in [\kappa]$ votes and $i \in [\kappa]$ evidences.
Although this implies a liveness violation, it is nevertheless a Nash equilibrium: the rational voters achieve the maximum reward voting for the genesis block, as their votes and evidences are included and rewarded on the chain.

Even though the rational voters violate the protocol rules by voting for the genesis block, it is not possible to punish them without risking punishment for honest voters under different circumstances.
This is due to the indistinguishability of the following two worlds for a late-coming client that observes the protocol after slot $\kappa+1$: (i) the world with honest leaders that broadcast the slot $i \in [\kappa]$ blocks $B_1, \ldots, B_{\kappa}$ in time, and (ii) the world where these leaders are adversarial and keep the blocks private until after slot $\kappa+1$.
In the first world, honest voters would vote for the blocks $B_1, \ldots, B_{\kappa}$, whereas in the second world, even the honest voters cannot vote for any block other than the genesis through slots $i \in [\kappa]$.
The indistinguishability of the two worlds enables the rational voters to pretend as if they are in world 2 while in world 1.
% An alternative to punishment would be rewarding the slot $t=1,\ldots,\kappa$ voters for voting for the latest block, \ie, the slot $B_t$ block.
% However, this gives the rewarding power back to the slot leaders, bringing back the earlier attacks in Sections~\ref{sec:solo-validators-simple,sec:solo-validators-extended}.
The example above is formalized and generalized to safety attacks in Appendix~\ref{sec:goldfish-liveness-attack} and demonstrates the difficulty of proving security with \emph{purely} rational validators that do not distinguish between any two action with the same payoff.
\vspace{-5 pt}
\subsection{Security of Goldfish under \NewMechanism}
\label{sec:security-under-new-mechanism}
% 
Since the two worlds above are indistinguishable for late-coming clients, witholding blocks is not an \emph{objectively} attributable fault via cryptographic proofs.
However, the current protocol observers can detect whether the blocks $B_1, \ldots, B_{\kappa}$ were published on time and raise an alarm if the blocks are withheld.
% in the case of attacks on the layer of \emph{social consensus} 
Such protocol violations for which there is agreement among the active protocol observers were categorized under the notion of \emph{intersubjectively attributable faults} and to a large extent allow the protocol to identify and punish the parties responsible for the violation~\cite{eigenblog,eigenpaper}.
Motivated by this observation, we assume that when a rational slot $t$ voter is indifferent between voting for different blocks in terms of payoff, it votes for the `correct' chain tip, \ie, the tip identified by the GHOST-Eph rule applied to its bvtree combined with the slot $t$ leader's proposed bvtree (\cf Section~\ref{sec:goldfish}).
Thus, rational validators are in fact assumed to be \emph{semi-rational} (semi-honest).
% indifferent between two actions in terms of payoff, they always choose the `honest' one required by the protocol.
% Intuitively, the rational validators would want to follow the protocol, unless there is a clear financial incentive to deviate.

We show our security result for non-colluding semi-rational validators formalized below.
% the Goldfish protocol satisfies security and reorg resilience in a Nash equilibri (\ie, equilibria, where deviation leads to a strict loss in payoff).
% We focus on a Goldfish variant with slots of length $4$~\cite[Section 3.2]{d2022goldfish}, where 
Recall that honest slot $t$ voters broadcast their votes at time $4t+1$ and merge their buffers into their bvtrees at time $4t+3$.
In contrast, semi-rational validators merely aim to maximize their payoffs subject to the following assumptions: 
% 
\begin{enumerate}
    \item Semi-rational validators are myopic: their goal at any slot is to maximize the payoff for the messages of that slot.
    \item As a slot $t$ voter, a semi-rational validators broadcasts at most a single vote, at or after $4t+1$, as casting multiple votes is a slashable offense (\cf Appendix~\ref{sec:slashing}).
    If it is indifferent between voting for multiple blocks at some time in $[4t+1,4t+3]$, it broadcasts a vote for the chain tip that was identified at time $4t+1$ by the GHOST-Eph rule applied to its bvtree combined with the proposed bvtree in its view.
    \item As a slot $t+1$ voter, it sends slot $t$ evidences only for the slot $t$ votes it observes at time $4t+2$.
    This is necessary to incentivize timeliness.
    \item As a slot leader, it acts honestly. 
    We consider a rational slot leader that commits to protocol deviations for higher profit as a Byzantine adversary (\cf Section~\ref{sec:credibility}).
\end{enumerate}
% 
We consider
% under rational solo (non-colluding) voters.
% $(\frac{1}{2},4\kappa)$-compliant executions, which in simple terms imply 
a non-colluding semi-rational majority among the awake validators at all times, the rest being adversarial.
The adversarial validators are always awake, and their number does not change as in the original sleepy network model~\cite{sleepy} (\cf Appendix~\ref{sec:goldfish-security}).
Finally, we assume that there are no financial transfers (\eg, bribery) among the validators.
% recovers its guarantees under rational validators:
% 
\begin{theorem}
\label{thm:goldfish-security}
Consider an execution of Goldfish in the synchronous sleepy network model.
Then, there exists a strict Nash equilibrium, where, all semi-rational voters attain the maximum possible payoff for all slots, and w.o.p., Goldfish is safe and live with transaction confirmation time of $2\kappa+2$ slots and satisfies reorg resilience: if a validator $v$ with block $B$ is recognized as the leader of a slot $t$ by the semi-rational validators at $4 t + 1$, then $\forall r \geq 4 t+3$, for all validators $v$, $B$ is in $v$'s canonical GHOST-Eph chain at time $r$.
Moreover, there is no strict Nash equilibrium, where Goldfish is not safe or live or reorg resilient with non-negligible probability.
\end{theorem}
% 
The proof is given in Appendix~\ref{sec:goldfish-security}.
It shows that the semi-rational voters are incentivized to broadcast timely votes in all strict Nash equilibria given the \newmechanism mechanism.
It then builds on the proof in \cite[Section 4]{d2022goldfish}.
%

==> staking_pools.tex <==
\section{Attacking in the Presence of Staking Pools}
\label{sec:staking-pools}
% 
In this section, we analyze the commitment attacks in the presence of staking pools.
%same attacks from Sections~\ref{sec:solo-validators-simple} and~\ref{sec:solo-validators-extended} in the presence of staking pools (Fig.~\ref{fig:simple_game_staking_pool_NANV}).
% A staking pool is defined as a set of colluding solo validators, thus having control over a set of attestors in each slot.
% According to the Ethereum protocol (\cf Section~\ref{sec:lmd-ghost-background}), each validator becomes a attestor in only one slot per epoch.
% However, validators from the same staking pool may serve as attestors at \emph{each} slot in the same epoch. 
% Controlling a set of validators in each slot of an epoch can affect the strategy of a rational staking pool against the attack.
A staking pool is defined as a group of colluding solo validators. Controlling a set of validators in each slot of an epoch can influence the strategy of a rational staking pool in response to an attack.
For instance, consider the simple game, where slot $t+1$ is adversarial. 
For analyzing this attack in the presence of solo validators, we only needed to consider the attestation reward that a solo validator receives for its vote in slot $t$.
However, in the presence of staking pools, we should consider the reward in both slots $t-1$ and $t$ as the staking pool may control attestors in both slots.
Indeed, if the adversary reorgs the block of slot $t$ in the simple game, the rewards of the staking pool for its slot $t-1$ votes are affected as well.

Despite the impact of staking pools on the response strategy to attacks, we establish the existence of a Nash equilibrium for the success of the simple game in the presence of staking pools in Appendix~\ref{sec:appendix-proof-simple-game-fixed}.
% and the existence of a SPNE for the success of the extended game in the presence of staking pools in Appendix~\ref{sec:appendix-proof-extended-game-fixed}. 
The analysis of the simple game in the presence of staking pools is intuitively illustrated in Figure~\ref{fig:simple_game_staking_pool}.
If a staking pool $P$ controls less than $\Wp$ attestors per slot, acting compliantly weakly dominates any other action in the simple game as shown in Fig.~\ref{fig:simple_game_staking_pool}.
On the other hand, if $P$ controls over $\Wp$ attestors\footnote{As of October 23, 2024, the largest staking pool is LIDO, holding $27.8\%<\Wp = \%40$ of the total Ethereum stake~\cite{lido}.} per slot, acting non-compliantly (voting for $B_{t}$) weakly dominates any other action in the simple game, even though following the adversarial action (voting for $B_{t-1}$) still remains weakly dominant. 

In long-range attacks, such as the extended attack, if validators coordinate their strategies, \ie, collude to form a single entity (e.g., a staking pool), compliance with the adversarial game rules would become a non-dominant strategy, leading to the mitigation of the attack. In the next section, we introduce the \emph{selfish mining-inspired attack}, where even colluding validators are incentivized to comply with the adversary. In the presence of rational staking pools, a selfish mining-inspired attack can threaten protocol liveness regardless of the size of the staking pools. However, the downside is that this attack requires a larger share of the stake.

% The existence of equilibria as in Note~\ref{note:extended_game_fixed_validator}, where the attestors achieve greater payoffs compared to the SPNE of the attack 
% % with greater payoffs 
% incentivizes them to 
% % coordinate their strategies or 
% collude as a single entity (\eg, a staking pool) to mitigate the attack. 
% % Second, following the extended game rules can dominate behaving non-compliantly for a player only if its subsequent players are payoff-maximizing validators. 
% % Even the existence of an honest minority (an honest slot leader) can affect the rational validators' strategy, resulting in the attack's failure.
% % 
% % An adversary faced with colluding attestors may refer to the \emph{selfish mining-inspired attack} in Appendix~\ref{sec:fixed-validator-set-selfish_mining_game}, which achieves adversarial success under more practical assumptions, albeit under higher requirements of control over slots. There, even colluding validators are incentivized to comply with the adversary.
% An adversary faced with colluding attestors may refer to the \emph{selfish mining-inspired attack} in Appendix~\ref{sec:fixed-validator-set-selfish_mining_game}, where even colluding validators are incentivized to comply with the adversary.
% % However, this attack requires higher adversarial control over slots.


% % Therefore, using the same analysis employed in the fixed validator set model (\cf Section~\ref{sec:fixed-validator-set-simple-game}, 
% % % \ref{sec:fixed-validator-set-extended-game}, 
% % and Appendix~\ref{sec:fixed-validator-set-selfish_mining_game}), we can establish the existence of Nash equilibria of the simple and selfish mining-inspired games in the presence of a staking pool \emph{with any size}, where the adversary succeeds.
% % % at no cost ($\br = 0$).
% % %D
% % This shows that the attacks could succeed even when the rational attestors collude.
% % Therefore, in addition to the attestation rewards of the staking pool for the slot $t$ votes, the simple-game attack also affects the rewards for the slot $t-1$ votes. 
% % As a staking pool may control part of the committee in both slots $t-1$ and $t$, we should consider the reward that a staking pool receives for its votes in both slots to analyze the attack.

\subsection{The Simple Game}
\label{sec:staking-pools-simple-game}
% 
The simple game and the adversarial action are the same as in Section~\ref{sec:simple-game} except that a staking pool, denoted by $P$ controls $m < \Wp$ attestors in both slots $t-1$ and $t$, and these attestors vote in a coordinated fashion.

\begin{theorem}
\label{thm:staking-pools-simple-game-theorem}
There exists a Nash equilibrium of the simple game in the presence of a staking pool with $m < \Wp$ members per slot, where the adversary succeeds at no cost ($\br = 0$).
\end{theorem}
% 
\begin{proof}
To analyze the simple game in the presence of staking pools, we calculate the pay-off matrix of the staking pool $P$. 
% Assume staking pool $P$ has $m$ attestors in each slot on average and 
Let $r$ represent the reward that each attestor receives for a correct and timely head vote included in the canonical chain.
Assume further that the slot $t$ leader is not part of $P$.
% The pay-off that a stake pool receives is equal to the sum of the head vote rewards that all its $2m$ attestors receive in both slots $t-1$ and $t$. 
The pay-off matrix of $P$ is presented in Table~\ref{table:pay-off-matrix_simple-game_staking-pool}. 
Each entry in the table is calculated as the sum of two components: The left component represents the attestation reward of slot $t-1$, while the right component represents the attestation reward of slot $t$. 
Overall, 4 different scenarios can occur:
\begin{itemize}
    \item $\mathbf{A-V_P}$ \textbf{corner:} Over $\Wp$ slot $t$ attestors and the staking pool $P$ vote for $B_t$.
    In this case, $B_t$ cannot be reorged by $B_{t+1}$, and the $m$ slot $t-1$ votes by $P$ are included in $B_t$.
    Thus, $P$ receives a total payoff of $rm$ for slot $t-1$. 
    However, since the slot $t$ votes of $P$ are non-compliant according to the game rule, the adversary $\mathcal{A}$ includes none of $P$'s votes in its slot $t+1$ block $B_A$. 
    Therefore, $P$'s reward for slot $t$ is equal to $0$.
    \item $\mathbf{A-NV_P}$ \textbf{corner:} Over $\Wp$ slot $t$ attestors vote for $B_t$, but the staking pool $P$ does not vote for $B_t$, instead voting for $B_t$'s parent.
    In this case, $B_t$ does not get reorged, and $P$ receives a total payoff of $rm$ for slot $t-1$. 
    As over $\Wp$ slot $t$ attestors have voted for $B_t$, $\mathcal{A}$ proposes its block on top of $B_t$.
    Therefore, $P$ does not receive any payoff for its slot $t$ votes for $B_{t-1}$, as they are not correct. 
    % Hence, $P$'s compliant slot $t$ votes are viewed as incorrect votes and cannot be included in the adversary's block. 
    % Therefore, $P$'s reward for slot $t$ is equal to $rm$.
    \item $\mathbf{NA-V_P}$ \textbf{corner:} $\Wp$ or less slot $t$ attestors vote for $B_t$, but the staking pool $P$ votes for $B_t$.
    Then, $B_t$ gets reorged, and $P$'s slot $t-1$ head vote reward, \ie, payoff, is equal to $0$.
    Since $P$'s slot $t$ votes are non-compliant, its payoff for slot $t$ is also equal to $0$.
    \item $\mathbf{NA-NV_P}$ \textbf{corner:} $\Wp$ or less slot $t$ attestors vote for $B_t$, and the staking pool $P$ does not vote for $B_t$. 
    Then, the attack is successful, and $\mathcal{A}$ reorgs $B_t$ with its block. 
    Since block $B_t$ gets reorged, $P$'s payoff for slot $t-1$ is equal to $0$, but it receives $rm$ reward for its compliant slot $t$ votes.
\end{itemize}
% 
\begin{table}
    \centering
    \caption{Pay-off matrix of a staking pool $P$ in the simple game. Let $V_P$ denote the events that the staking pool $P$ votes for $B_t$. Let $A$ denote the event that over $\Wp$ slot $t$ attestors vote for $B_t$.}
    \begin{tabular}{|c|c|c|}
        \hline
          & $V_P$ & $NV_P$ \\
         \hline
         $A$ & $mr+0$ & $mr+0$ \\
         \hline
         $NA$ & $0+0$ & $0+mr$\\
         \hline
    \end{tabular}
    \label{table:pay-off-matrix_simple-game_staking-pool}
\end{table}
% 
As can be seen in Table~\ref{table:pay-off-matrix_simple-game_staking-pool}, similar to solo validators, voting for the empty block is a weakly dominant strategy for staking pools. This indicates that if rational validators, whether solo validators or staking pools, constitute over $W-\Wp$ of the committees, the simple attack would be successful. 
\end{proof}

\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in]{Pic3.jpg}
        \caption{$A$, $V_P$}
        \label{fig: simple_game_staking_pool_AV}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in]{Pic4.jpg}
        \caption{$A$, $NV_P$}
        \label{fig: simple_game__staking_pool_ANV}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in]{Pic5.jpg}
        \caption{$NA$, $V_P$}
        \label{fig: simple_game__staking_pool_NAV}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in]{Pic6.jpg}
        \caption{$NA$, $NV_P$}
        \label{fig:simple_game_staking_pool_NANV}
    \end{subfigure}%
    \caption{The simple game in the presence of staking pool $P$. Let $V_P$ and $NV_P$ denote the events that the staking pool $P$ votes and does not vote for $B_t$, respectively. Let $A$ denote the event that over $\Wp$ slot $t$ attestors vote for $B_t$. Conversely, $NA$ denotes the event that $\Wp$ or less slot $t$ attestors vote for $B_t$. The green tick and the red cross represent whether a head vote receives or does not receive a reward, respectively.}
\end{figure*}

\begin{note}
There are Nash equilibria, similar to those in Section~\ref{sec:solo-validators-simple}, where the adversary $\mathcal{A}$ is not successful. 
However, $\mathcal{A}$ can again ensure its success in \emph{all} Nash equilibria by offering an $\epsilon/W$ amount of bribe to each slot $t$ attestor to vote for $B_{t-1}$.
\end{note}

\begin{note}
If the staking pool $P$ controls over $\Wp$ attestors per slot, payoff of the $NA - V_P$ corner becomes $mr+0$ for $P$ in Table~\ref{table:pay-off-matrix_simple-game_staking-pool}.
Then, voting for block $B_t$ at slot $t$ weakly dominates voting for $B_{t-1}$ for $P$, given any actions by the other attestors.
If $P$ votes for $B_t$, $\mathcal{A}$ cannot reorg $B_t$ with its block $B_A$, \ie, is unsuccessful.
\end{note}


\subsection{The Extended Game}
\label{sec:staking-pools-extended-game}
% 
The extended game and the adversarial action are the same as in Section~\ref{sec:solo-validators-extended} except that a staking pool, denoted by $P$ controls $m < \Wp$ attestors in all slots, and these attestors vote in a coordinated fashion. 
We again assume that the staking pool does not control any of the leaders for slots in $[p]$.
% 
\begin{theorem}
\label{thm:staking-pools-extended-game-theorem}
There exists a subgame perfect Nash equilibrium of the extended game in the presence of a staking pool with $m < \Wp$ members per slot, where the adversary succeeds at no cost ($\br = 0$) and violates safety and liveness.
\end{theorem}
% 
Proof of Theorem~\ref{thm:staking-pools-extended-game-theorem} follows the same outline as the proof of Theorem~\ref{thm:repeated-game-theorem} and presented in Appendix~\ref{sec:appendix}.
Since the staking pool controls less than $\Wp$ attestors per slot, it has the same payoff table for the attestation rewards of each slot $i \in [p]$ as Tables~\ref{table:payoff_matrix-repeated_game_p} and~\ref{table:payoff_matrix-repeated_game_i}.

\begin{note}
There are subgame perfect Nash equilibria, similar to those in Section~\ref{sec:solo-validators-extended}, where the adversary $\mathcal{A}$ is not successful.
However, $\mathcal{A}$ can again ensure its success in \emph{all} subgame perfect Nash equilibria by offering an $\epsilon/pW$ amount of bribe to each slot $t$ attestor to send compliant votes.
\end{note}

\begin{note}
If the staking pool $P$ controls over $\Wp$ attestors per slot, it can ensure that sending a non-compliant vote weakly dominates any other action at each subgame $\texttt{G}^\val_i$, $i \in [p]$ similar to Section~\ref{sec:staking-pools-simple-game}.
\end{note}

% 
% A rational staking pool $P$ can prevent the adversary $\mathcal{A}$ from succeeding in the ex game. 
% Recall that in the extended game, the attack succeeds if the empty blocks $B^e_{i}$, $i \in [p]$, enter and stay in the canonical chain after slot $p$, and the attack fails otherwise.
% The payoff matrix of a staking pool $P$ in the extended game is presented in Table~\ref{table:pay-off-matrix_normal-extended-game_staking-pool}. 
% In the table, we have considered the attack failure to be equivalent to the worst-case scenario for the adversary, where non-empty blocks $B_{i}$, $i \in [p]$, enter and stay in the canonical chain.
% % 
% \begin{table}
%     \centering
%     \caption{Pay-off matrix of a staking pool $P$ in the extended version of the attack. Let $\mathcal{H}_P$ and $\mathcal{A}_P$ denote the events that the staking pool $P$ follows the honest protocol and the adversary's game rule, respectively.}
%     \begin{tabular}{|c|c|c|}
%         \hline
%           & $\mathcal{H}_P$ & $\mathcal{A}_P$ \\
%          \hline
%          Attack fails. & $pmr$ & $mr$ \\
%          \hline
%          Attack succeeds. & $mr$ & $(p+1)mr$\\
%          \hline
%     \end{tabular}
%     \label{table:pay-off-matrix_normal-extended-game_staking-pool}
% \end{table}
% % 
% Following the game rule is not a Nash equilibrium for the staking pool $P$, indicating that there is no Nash equilibrium, where the adversary succeeds.

% In the next section, we introduce the advanced version of the extended game that can be applied in the presence of staking pools. 
% The advanced extended game, which resembles the selfish mining attack, reduces the security of the LMD GHOST fork choice rule to the security of the predictable longest-chain fork choice rule.
% Suppose $\Wp / p = 1/4$, $p = 10$ and $P$ votes for the blocks $B_i$, $i \in [p]$.
% In this case, the adversary cannot reorg the blocks $B_1, \ldots, B_k$, even if all other attestors follow adversary's game, where $k$ is the largest number in $[p]$ such that $(p-k)m \geq \Wp$.
% Then, $P$ gains an attestation reward of $k m r$, which is larger than the maximum attestation reward it could get $(m r)$ when $\mathcal{A}$ succeeds.
% Therefore, there is no Nash equilibrium, where the adversary succeeds.
% 
% If the adversary controls enough attestors each slot to offset $P$'s votes (more specifically, the votes of the largest staking pool), it can again successfully do the extended attack in Section~\ref{sec:repeated-game-adversarial-action}.
% The analysis is the same as in Section~\ref{sec:repeated-game-analysis}.

\subsection{The Repeated Simple Game}
\label{sec:advanced_extended_game}
% 
The repeated simple game in the presence of staking pools starts at the beginning of some slot $t$.
We normalize slot $t-1$ to be slot $0$.
It has the adversary, attestors of the slots in $[p]$, and the leaders of the slots in $[p+1]$ as its players.
% The leader of slot $p+1$ is adversarial.
% The number of adversarial slots within slot range $[1, p+1]$ is greater than or equal to the number of non-adversarial slots.
Let $N_\mathcal{A}$ and $N_\mathcal{NA}$ denote the number of adversarial slots and non-adversarial slots within the slot range $[p+1]$.
The repeated simple game requires the condition $N_\mathcal{A} \ge N_\mathcal{NA}$.
% Let $B_0$ denote the block at the tip of the canonical LMD GHOST chain at the end of slot $0$.
Let $s_i$ and $B^\mathcal{A}_i$, $i \in \{1, \ldots, N_\mathcal{A}\}$, denote the $i^\text{th}$ adversarial slot within slot range $[p+1]$ and its corresponding block, respectively.
The attack \emph{succeeds} if the canonical LMD-GHOST chain at the end of slot $p+1$ is a sequence of blocks $B^\mathcal{A}_{i}$, $i \in \{1, \ldots, N_\mathcal{A}\}$.
The attack \emph{fails} otherwise.
The game ends, and the payoffs are realized at the end of slot $p$ at time $3p+3$.

\subsubsection{Adversary's Action}
\label{sec:advanced-extended-game-adversarial-action}

We next describe the adversary's action. 
% 
\begin{definition}[Adversary's Action for the Advanced Extended Game]
\label{def:adversary-action-extended-2}
    Before slot $1$ starts, the adversary $\mathcal{A}$ generates a proof asserting its leadership in the adversarial slots within the range $[p+1]$.
    Then, for the slots $s_i-1$, $i \in \{1, \ldots, N_\mathcal{A}\}$, it sets the game rule $\texttt{Game}_i$ as follows: 
    The attestors of slot $s_i-1$ should refrain from publishing their votes at time $3(s_i-1)+1$. They should later vote for block $B^\mathcal{A}_{i-1}$ that will be published by the adversary at a point in the time range $[3p, 3(p+1)+1]$\footnote{The time range is after all the non-adversarial blocks within $[p]$ have been published and before the voting time of slot $p+1$ starts.}.
    Here, $B^e_0 = B_0$.
    
    The game does not specify any rules for the attestors of the remaining slots.

    At the start of slot $p$, when all the non-adversarial blocks within $[p]$ have been published, the adversary $\mathcal{A}$ takes the following sequential action for $i \in \{1, \ldots, N_\mathcal{A}\}$:
    % 
    \begin{itemize}[leftmargin=*]
        \item It publishes block $B^\mathcal{A}_{i-1}$ for the attestors of slot $s_i-1$.
        \item It collects the votes submitted by the attestors of slot $s_i-1$ for block $B^\mathcal{A}_{i-1}$ and inserts them into the block $B^\mathcal{A}_{i}$ as compliant votes.
    \end{itemize}
    Before time $3(p+1)+1$, the adversary publishes the sequence of blocks $B^\mathcal{A}_{i}$, $i \in \{1, \ldots, N_\mathcal{A}\}$ for all the validators.
\end{definition}

\subsubsection{Analysis}
\label{sec:advanced-extended-game-analysis}
%
Let the non-adversarial fork be the fork that is published by non-adversarial validators by the end of slot $p$ and the adversarial fork be the sequence of blocks $B^\mathcal{A}_{i}$, $i \in \{1, \ldots, N_\mathcal{A}\}$. If the attestors of all slots $s_i-1$, $i \in \{1, \ldots, N_\mathcal{A}\}$ are incentivized to follow the adversary's game rule rather than the honest protocol, the weights of the non-adversarial fork and the adversarial fork at time $3(p+1)+1$ will be equal to $N_\mathcal{NA}W$ and $N_\mathcal{A}W+W_p$, respectively. As $N_\mathcal{A}\ge N_\mathcal{NA}$, the weight of the adversarial fork will be higher, and the attack will succeed. In the following theorem, we show that a rational staking pool is incentivized to follow the game rule.
% 
\begin{theorem}
\label{thm:repeated-game-theorem-2}
There exists a Nash equilibrium of the repeated simple game, where the adversary succeeds at no cost ($\br = 0$).
\end{theorem}

\begin{proof}
    The payoff matrix of a staking pool $P$ in the repeated simple game is presented in Table~\ref{table:pay-off-matrix_advanced-extended-game_staking-pool}.
    \begin{table}
    \centering
    \caption{Pay-off matrix of a staking pool $P$ in the repeated simple game. Let $\mathcal{H}_P$ and $\mathcal{A}_P$ denote the events that the staking pool $P$ follows the honest protocol and follows the adversarial game rule, respectively. Let $\text{fork}_\mathcal{A}$ denote that the adversarial fork at time $3(p+1)+1$ outweighs the non-adversarial fork. Conversely, $\text{fork}_\mathcal{NA}$ denotes that the non-adversarial fork at time $3(p+1)+1$ outweighs the adversarial fork.}
    \begin{tabular}{|c|c|c|}
        \hline
          & $\mathcal{H}_P$ & $\mathcal{A}_P$ \\
         \hline
         $\text{fork}_\mathcal{NA}$ & $N_\mathcal{NA}mr$ & $N_\mathcal{NA}mr$ \\
         \hline
         $\text{fork}_\mathcal{A}$ & $0$ & $N_\mathcal{A}mr$\\
         \hline
    \end{tabular}
    \label{table:pay-off-matrix_advanced-extended-game_staking-pool}
\end{table}
Following the game rule weakly dominates following the honest protocol. Therefore, a rational staking pool follows the game rule, resulting in the adversary's success.
\end{proof}

The repeated simple game, which resembles the selfish mining attack, reduces the security of the LMD GHOST fork choice rule to the security of the predictable longest-chain fork choice rule.

==> tendermint_new_mechanism.tex <==
\section{The New Mechanism on Tendermint}
\label{sec:new-mechanism-tendermint}

In this section, we define and show an analogue of reorgs (as well as liveness attacks), which can affect Tendermint under rational validators if it does not use a decentralized reward mechanism.
We then prove that the new reward mechanism, applied to Tendermint ensures security under rational validators.

\subsection{Tendermint in a Nutshell}

Tendermint~\cite{tendermint} is an accountably-safe PBFT-style SMR consensus protocol that satisfies security under partial synchrony if over $2/3$ of its validators are honest.
It proceeds in phases called \emph{heights}, during which the validators attempt to finalize a unique block at that height.
Heights are in turn divided into \emph{rounds}, each with a unique leader.
Rounds consist of three steps: proposal, prevote and precommit, each with duration $\Delta = 1$.
At the start of the proposal step, the round leader broadcasts a proposal $\langle \mathsf{Proposal}, h, r, B, vr \rangle$ containing the height number $h$, the round number $r$, the proposed block $B$, and a \emph{validRound} number $vr$.
At the prevote step, each validator $\val$ broadcasts a prevote $\langle \mathsf{Prevote}, h, r, \text{hash}(B) \rangle$ for either the proposed block $B$, or a special \emph{nil} value ($B = \bot$), as determined by its view of the protocol messages.
If $\val$ receives $2f+1$ prevotes for a block $B$ (or $\bot$) by the start of the precommit step, it broadcasts a precommit $\langle \mathsf{Precommit}, h, r, \text{hash}(B) \rangle$ for $B$ (or $\bot$).
Finally, a validator or a client \emph{finalizes} a block $B \neq \bot$ for height $h$ upon observing $2f+1$ precommits with height $h$ for the block.
If no non-nil block is finalized after a round, the round number is incremented, and the validators enter a new round.
% For more details, \cf Appendix~\ref{sec:appendix-tendermint-overview-continued}.

Each validator $\val$ keeps track of four parameters: lockedRound, lockedValue, validRound and validValue.
The lockedValue and lockedRound respectively represent the latest block and its round number (initially `$-1$') such that $\val$ sent a precommit for the block.
The validValue and validRound respectively represent the latest block and its round number (initially $-1$) such that $\val$ has received $2f+1$ distinct prevotes for the block ($\text{validRound} \geq \text{lockedRound}$ since $\val$ must have seen $2f+1$ prevotes for a block before sending a precommit for it).
There are three conditions \emph{either} of which must be satisfied for $\val$ to send a prevote for a proposed block $B \neq \bot$: (i) if $\val$'s lockedValue is $-1$ ($\val$ is not locked on any block), or (ii) if $B$ is the same as $\val$'s lockedValue (whenever $\val$ is locked on a block), or (ii) if the value $vr$ in the proposal message is at least as large as $\val$'s lockedValue, and $\val$ has received $2f+1$ round $vr$ prevotes for $B$.
If none of the voting rules is satisfied, $\val$ sends a prevote with the \emph{nil} value.
If $\val$ with validRound $vr$ is the round leader, it proposes a new block if $vr = -1$ and its validValue (block) if $vr > -1$, both with validRound $vr$.

% Each validator $\val$ keeps track of four parameters: lockedRound, lockedValue, validRound and validValue.
% The lockedValue and lockedRound respectively represent the latest block and its round number (initially `$-1$') such that $\val$ sent a precommit for the block.
% The validValue and validRound respectively represent the latest block and its round number (initially $-1$) such that $\val$ has received $2f+1$ distinct prevotes for the block ($\text{validRound} \geq \text{lockedRound}$ since $\val$ must have seen $2f+1$ prevotes for a block before sending a precommit for it).
% There are three conditions \emph{either} of which must be satisfied for $\val$ to send a prevote for a proposed block $B \neq \bot$: (i) if $\val$'s lockedValue is $-1$ ($\val$ is not locked on any block), or (ii) if $B$ is the same as $\val$'s lockedValue (whenever $\val$ is locked on a block), or (ii) if the value $vr$ in the proposal message is at least as large as $\val$'s lockedValue, and $\val$ has received $2f+1$ round $vr$ prevotes for $B$.
% If none of the voting rules is satisfied, $\val$ sends a prevote with the \emph{nil} value.
% If $\val$ with validRound $vr$ is the round leader, it proposes a new block if $vr = -1$ and its validValue (block) if $vr > -1$, both with validRound $vr$.
% % For the full protocol description, see the paper~\cite{tendermint}.

\subsection{Tendermint under Rational Validators}

Tendermint as implemented for Cosmos chains rewards block proposers for including precommits from the previous height in proportion to the number of included precommits.
If any of the fees accrued by the proposal remains on the table, it is distributed evenly among \emph{all} validators, not just those whose precommits were included~\cite{tendermint_reward}.
% Tendermint with a \emph{centralized} reward mechanism, \eg, one that enables the height $h$ block to determine the rewards for the height $h-1$ prevotes and precommits, would be susceptible to simple and extended attacks similar to those in Section~\ref{sec:solo-validators-simple} and~\ref{sec:solo-validators-extended}.
% Such attacks would imply existence of equilibria, where no block is finalized for arbitrarily many rounds in a row during a height\footnote{However, unlike in Section~\ref{sec:solo-validators-extended}, the attacks would not be able to \emph{reorg} finalized Tendermint blocks.}.
Therefore, there is no explicit incentive ingrained into the protocol to reward an individual validator for a timely prevote or precommit.
This could result in \emph{tragedy of commons}, where each validator expects the others to finalize a block with their precommits; so that it can receive a payoff from the next block without sending a precommit.
% To avoid these attacks,
In contrast, if the protocol were to reward validators for timely precommits as in LMD GHOST, due to attacks similar to those in Section~\ref{sec:solo-validators-extended}, honest proposals would fail to gather sufficiently many precommits to be finalized in the presence of rational validators. 
Then, under both reward mechanisms and rational validators, Tendermint might consistently fail to finalize the blocks proposed by honest validators (even under synchronous network conditions), thus eventually lose its liveness altogether.
The failure to finalize an honest proposal despite synchrony would be analogous to reorgs, since the transactions and MEV opportunities within these honest proposals can later be captured by adversarially proposed and finalized blocks.

\subsection{New Reward Mechanism for Tendermint}
To avoid these attacks, we introduce a new decentralized reward mechanism akin to the Ethereum one.
Consider Tendermint run by $n = 3f+1$ validators.
We denote a round $r$, height $h$ message (proposal, prevote or precommit) by the term $(r,h)$ message.
As in Ethereum, the new mechanism relies on evidences sent by validators to reward prevotes and precommits.
Let $\langle \mathsf{Proposal}, h, r, B, vr \rangle$, $B \neq \bot$, denote the proposal received by a validator $\val$ from the round $r$ leader if it receives any proposal before the prevote step.
% 
% \begin{itemize}

\smallskip
\noindent
% \item 
\textbf{Prevote Evidence:}
While sending an $(r,h)$ precommit, $\val$ signs the $(r,h)$ prevote by a validator $\val'$ for a block $B'$ (including $B' = \bot$), if (i) $\val$ also sent an $(r,h)$ prevote for $B'$, or (ii) if $B' = \bot$, $\val$ sent an $(r,h)$ prevote for $B$, and $\val$ has received $2f+1$ $(r',h)$ prevotes with $r' \geq vr$ for a non-nil, round $r'$ block $B'' \neq B$ from $\val'$.
These prevotes forwarded by $\val'$ \emph{attest} to the fact that $\val'$ is locked on the non-nil block $B'' \neq B$ from round $r' \geq vr$, and this is why $\val'$ sent a prevote for a nil block $B' = \bot$. 
Signature of $\val$ on the prevote of $\val'$ is called an $(r,h)$ prevote evidence.

% \item 
\smallskip
\noindent
\textbf{Precommit Evidence:}
While sending an $(r = 1, h)$ prevote, $\val$ signs the $(r',h' = h-1)$ precommit by a validator $\val'$ for a block $B'$ (including $\bot$), if (i) $\val$ also sent an $(r', h')$ precommit for $B'$, or if (ii) $\val$ has received $2f+1$ $(r', h')$ prevotes for $B'$ from $\val'$ by the end of the $(r', h')$ precommit step.
Here, $r'$ is the last round of height $h-1$.
Note that the $2f+1$ $(r', h')$ prevotes for $B'$ from $\val'$ are to justify the precommit of $\val'$ for $B'$.
While sending an $(r>1, h)$ prevote, $\val$ signs the $(r' = r-1, h' = h)$ precommit by a validator $\val'$ for a block $B'$ (including $\bot$), if (i) $\val$ also sent a $(r', h')$ precommit for $B'$, or if (ii) $\val$ has received $2f+1$ $(r', h')$ prevotes for $B'$ from $\val'$ by the end of the $(r', h')$ precommit step.
Signature of $\val$ on the precommit of $\val'$ is called an $(r',h')$ precommit evidence.
% \end{itemize}
% 

A validator gains an attestation reward for its $(r,h)$ prevote (precommit) for a block $B$, once the vote is included in a finalized $(r',h')$ block $B'$, and it is \emph{correct} and \emph{timely}, redefined as follows:
% 
% \begin{itemize}
% \item 

\smallskip
\noindent
\textbf{Correctness:}
The $(r,h)$ prevote (precommit) is correct if $h < h'$, or $h = h'$ and $r < r'$.
    % \item 

\smallskip
\noindent
\textbf{Timeliness:}
The $(r,h)$ prevote (precommit) is timely if there are $2f+1$ unique $(r,h)$ prevote (precommit) evidences for it in $B'$.
% \end{itemize}

% As in Section~\ref{sec:slashing}, rational validators do not engage in accountably detectable protocol violations.
% For example, a rational validator does not send an $(r,h)$ precommit for a nil block, and then later attest that it was locked on (sent an $(r,h)$ precommit for) a non-nil block.

\subsection{A Liveness Attack on Tendermint}
\label{sec:appendix-proof-tendermint-bad}

Since Tendermint is $(f+1)$-accountably safe (\cf Section~\ref{sec:slashing}), and the rational validators do not violate the slashing rules, the protocol satisfies safety.
However, given rational validators, the new reward mechanism cannot ensure liveness in all Nash equilibria due to the indistinguishability of late-released messages and those broadcast at the correct time, yet included in later blocks.
We next show a Nash equilibrium with no liveness, where the rational validators create evidences for each others' messages, but withhold those messages and evidences for a long sequence of rounds.
Once the prevotes and precommits are broadcast, their corresponding evidences are included in a future block, and the rational validators are rewarded, despite stalling finality.

\subsubsection{Attack Game}
Consider an execution of Tendermint with $n = 3f+1$ validators.
The game starts at the beginning of round $r = 1$ of some height $h$.
It has the adversary and the rational validators as its players.
Out of the $3f+1$ validators, $f$ are adversarial, $m < f+1$ are honest, and the remaining ones are rational.
The first $m$ rounds of height $h$ have the honest validators as leaders.
The payoffs are as in Section~\ref{sec:simple-game} and realized at the end of round $m+1$.
The actions available to the players for any $(r,h)$ are:
% 
% \begin{itemize}
    % \item 

\smallskip
\noindent
(1) A rational leader proposes at most a \emph{single} $(r,h)$ block.
    % \item 
    
\smallskip
\noindent
(2) A rational validator sends at most a \emph{single} $(r,h)$ prevote (precommit) for any block or the nil value.
    % \item 

\smallskip
\noindent
(3) Adversarial validators can deviate from the protocol arbitrarily.
% \end{itemize}

Although the honest action for the validators is to broadcast their prevotes and precommits at the beginning of the respective steps, they can release these messages at a later time.

\begin{theorem}
\label{thm:tendermint-bad-equilibrium}
There exists a Nash equilibrium of the game above, where liveness is violated.
\end{theorem}
% 
\begin{proof}
We omit the mention of heights in the proof below as the game happens during height $h$.
Consider the following action profile followed by the adversarial and rational validators (\ie, all validators other than the leaders of the first $m$ rounds).
% \begin{itemize}
    % \item 

\smallskip
\noindent
(1) For each $r \in [m]$, every validator $\val$ creates round $r$ prevotes and precommits for \emph{nil} blocks.
% \item 

\smallskip
\noindent
(2) With each round $r \in [m]$ precommit, $\val$ creates $r$ prevote evidences for the $r$ prevotes by all non-honest validators.
    % \item 

\smallskip
\noindent
(3) With each round $r=2, \ldots, m$ prevote, $\val$ creates $r-1$ precommit evidences for the $r-1$ precommits by all non-honest validators.
% \end{itemize}

All of these prevotes, precommits and evidences from rounds $r \in [m]$ are kept private and are not broadcast to the honest validators and clients until round $m+1$.
Note that none of the honest validators update its lockedRound, lockedValue, validRound and validValue, and each of them proposes a new block $B$ that gathers only $m<f+1$ votes from the other honest validators.

Once round $m+1$ starts, all withheld messages are broadcast to the honest validators and clients.
Then, the round $m+1$ proposer proposes a block containing the previously withheld evidences, and for which all validators send prevotes and precommits, thus finalizing the block.
Therefore, by the end of round $m+1$, each validator other than the leaders of the first $m$ rounds achieves a payoff of $r m$.
As this is the largest payoff any rational validator can achieve throughout the game, this constitutes a Nash equilibrium, where liveness is violated since no block is finalized for height $h$ for the first $m$ rounds despite synchrony and honest leaders.
\end{proof}

The attack above is due to the rational validators' indifference between broadcasting their messages at the time suggested by the protocol and doing so at a later time, when they all engage in the same late-release attack.
However, taking such collective actions requires coordination among validators, making it unlikely in practice.
A definitive solution to coordinated attacks would be to empower the round leaders, which were notably left out of the collective strategy in the game above, to determine who voted for the previous round's block.
Albeit, this brings back the earlier attacks.

\subsection{Analysis}
\label{sec:new-mechanism-tendermint-analysis}

In real-world deployments of protocols, there are altruistic validators who do not simply engage in any protocol deviation that offers a higher payoff in the short run.
Such honest validators can serve as the anchor needed by the new reward mechanism to incentivize the timely broadcast of messages.
Therefore, we reanalyze the mechanism in the presence of $f+1$ \emph{honest} validators\footnote{As an honest minority is already needed to avoid data availability attacks, another potential cause of liveness violations that cannot be accountably detected or punished~\cite{babylon}, the assumption of $f+1$ honest validators is ingrained into any incentive analysis of PBFT-style protocols.} (recall that neither Ethereum's nor Tendermint's old mechanisms can ensure security under an honest minority).
% We merely continue this theme in the analysis below.
In the result below, we assume \emph{myopic} validators, whose goal at every round is to maximize the payoff for the messages of that round.
% 
\begin{theorem}
\label{thm:tendermint-good-equilibrium}
Consider Tendermint with $3f+1$ validators, where $f$ validators are adversarial, $f+1$ validators are honest, and the remaining ones are rational.
Then, the protocol satisfies liveness and reorg resilience in all Nash equilibria.
\end{theorem}
% 
%Proof of Theorem~\ref{thm:tendermint-good-equilibrium} is in Appendix~\ref{sec:appendix-proof-tendermint-good} and follows from rational validators voting timely to gather evidences from honest validators.
%
\begin{proof}[Proof of Theorem~\ref{thm:tendermint-good-equilibrium}]
No rational validator $\val$ can gain a reward for its $(r,h)$ prevote or precommit without an honest validator creating an $(r,h)$ prevote or precommit evidence for $\val$'s message.

Consider the first round $r$ of a height $h$ with an honest leader $L$.
Towards contradiction, suppose less than $2f+1$ prevotes are broadcast for $L$'s block $B$ at the prevote step.
Let $\langle \mathsf{Proposal}, h, r, B, vr \rangle$ denote $L$'s proposal.
All honest validators broadcast a prevote for $B$; because if any honest validator was locked on any block $B' \neq B$ from a round $r' \geq vr$, then $L$'s validRound would be at least $r'$ (and if $r' = vr$, $B$ would have been $B'$), \ie, a contradiction.
Thus, suppose a rational validator $\val$ did not vote for $B$, instead sending a prevote for nil.
Then, to gain any payoff, it must have broadcast $2f+1$ round $r' \geq vr$ prevotes for a block $B' \neq B$, which $\val$ claims to have locked on at round $r'$.

Now, suppose $\val$ sent a round $r'$ precommit for some block $B''$.
If $B'' = B'$, for $\val$ to gain any payoff for its round $r'$ precommit, either an honest validator must have sent a round $r'$ precommit for $B'$ or $\val$ must have sent the $2f+1$ $r'$ prevotes to at least one honest validator by the end of the round $r'$ precommit step, which in turn would have broadcast these votes to all other validators.
In either case, $L$'s validRound would be at least $r'$ (and if $r' = vr$, $B$ would have been $B'$), \ie, contradiction.
On the other hand, if $B'' \neq B$, either $\val$ must have forgone the reward for its round $r'$ precommit (which is a contradiction with the myopic rationality assumption), or there must be $2f+1$ round $r'$ prevotes for $B''$; as otherwise, no honest validator can sent a round $r'$ precommit for $B''$ and $\val$ cannot broadcast $2f+1$ $r'$ prevotes for $B''$ to get rewarded.
However, this is a contradiction, since then $\val$ cannot show $2f+1$ round $r'$ prevotes for $B'$ in round $r$.

Finally, since all honest validators observe $2f+1$ prevotes for $B$, they broadcast precommits for $B$.
Moreover, as there are less than $2f+1$ round $r$ prevotes for any other block $B' \neq B$, to gain a reward for its round $r$ precommit, each rational validator broadcasts an $r$ precommit for $B$.
Thus, $B$ becomes finalized, implying the liveness and reorg resilience of the protocol.
\end{proof}
